DITTO: Data-efficient and Fair Targeted Subset Selection for ASR Accent Adaptation

State-of-the-art Automatic Speech Recognition (ASR) systems are known to exhibit disparate performance on varying speech accents. To improve performance on a specific target accent, a commonly adopted solution is to finetune the ASR model using accent-specific labeled speech. However, acquiring large amounts of labeled speech for specific target accents is challenging. Choosing an informative subset of speech samples that are most representative of the target accents becomes important for effective ASR finetuning. To address this problem, we propose DITTO (Data-efficient and faIr Targeted subseT selectiOn) that uses Submodular Mutual Information (SMI) functions as acquisition functions to find the most informative set of utterances matching a target accent within a fixed budget. An important feature of DITTO is that it supports fair targeting for multiple accents, i.e. it can automatically select representative data points from multiple accents when the ASR model needs to perform well on more than one accent. We show that DITTO is 3-5 times more label-efficient than other speech selection methods on the IndicTTS and L2 datasets.

==> tables/indic-2.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|l|l|l|l|l|l|l|l||l|}
\hline
\textbf{Targeted} & \textbf{metric} & \multicolumn{1}{c}{\textbf{pretrain}} & \textbf{random} & \textbf{entropy} & \textbf{diversity} & \textbf{FacLoc} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FL2MI}  \\
Ass-Mal           & Ass-WER         & \multicolumn{1}{c}{27.06}             & 20.4            & 24.85            &                    & 20.12           & 21.05           & 21.11           & \textbf{19.68}  \\
Ass-Mal           & Mal-WER         & \multicolumn{1}{c}{19.49}             & 16.21           & 16.78            &                    & 18.74           & 17.47           & \textbf{13.97}  & 14.67           \\
Ass-Mal           & selected \%s    &                                       & 17.8\% - 10.9\% & 1.9\% - 8.6\%    &                    & 16.2\% - 8.7\%  & 15.2\% - 4.4\%  & 24.7\% - 75.3\% & 50.6\% - 49.4\% \\
Ass-Mal           & fairness\_\%    &                                       & 7.8             & 0.7              &                    & 5.6             & 2.7             & 74.4            & \textbf{100}    \\
Ass-Mal           & mean\_WER       &                                       & 18.3            & 20.82            &                    & 19.43           & 19.26           & 17.54           & \textbf{17.18}  \\
Mal-Raj           & Mal-WER         & \multicolumn{1}{c}{19.49}             & 16.21           & 16.78            &                    & 18.74           & 17.47           & 15.74           & \textbf{15.04}  \\
Mal-Raj           & Raj-WER         & \multicolumn{1}{c}{21.88}             & 16.19           & 15.81            &                    & 15.92           & 16.09           & \textbf{13.3}   & 14.26           \\
Mal-Raj           & selected \%s    &                                       & 10.9\% - 8.5\%  & 8.6\% - 12.4\%   &                    & 8.7\% - 8.9\%   & 4.4\% - 7.5\%   & 7.6\% - 92.4\%  & 21.9\% - 78.1\% \\
Mal-Raj           & fairness\_\%    &                                       & 3.7             & 4.3              &                    & 3.1             & 1.3             & 28.1            & \textbf{68.4}   \\
Mal-Raj           & mean\_WER       &                                       & 16.2            & 16.3             &                    & 17.33           & 16.78           & \textbf{14.52}  & 14.65           \\
Ass-Raj           & Ass-WER         & \multicolumn{1}{c}{27.06}             & \textbf{20.4}   & 24.85            &                    & 20.12           & 21.05           & 25.63           & \textbf{21.21}  \\
Ass-Raj           & Raj-WER         & \multicolumn{1}{c}{21.88}             & 16.19           & 15.81            &                    & 15.92           & 16.09           & \textbf{13.29}  & 14.34           \\
Ass-Raj           & selected \%s    &                                       & 17.8\% - 8.5\%  & 1.9\% - 12.4\%   &                    & 16.2\% - 8.9\%  & 15.2\% - 7.5\%  & 0.0\% - 100.0\% & 25.5\% - 74.5\% \\
Ass-Raj           & fairness\_\%    &                                       & 6.1             & 0.9              &                    & 5.8             & 4.6             & 0               & \textbf{76}     \\
Ass-Raj           & mean\_WER       &                                       & 18.3            & 20.33            &                    & 18.02           & 18.57           & 19.46           & \textbf{17.77}  \\
Ass-Man           & Ass-WER         & \multicolumn{1}{c}{27.06}             & 20.4            & 24.85            &                    & 20.12           & 21.05           & 17.08           & \textbf{17.05}  \\
Ass-Man           & Man-WER         & \multicolumn{1}{c}{53.08}             & 42.55           & 47.22            &                    & 42.42           & \textbf{40.73}  & 44.57           & 42.91           \\
Ass-Man           & selected \%s    &                                       & 17.8\% - 13.6\% & 1.9\% - 3.8\%    &                    & 16.2\% - 12.9\% & 15.2\% - 23.9\% & 97.8\% - 2.2\%  & 92.6\% - 7.4\%  \\
Ass-Man           & fairness\_\%    &                                       & 9.7             & 0.3              &                    & 8.4             & 14.5            & 8.6             & \textbf{27.4}   \\
Ass-Man           & mean\_WER       &                                       & 31.48           & 36.03            &                    & 31.27           & 30.89           & 30.82           & \textbf{29.98}  \\
Man-Raj           & Man-WER         & \multicolumn{1}{c}{53.08}             & 42.55           & 47.22            &                    & \textbf{42.42}  & 40.73           & 48.91           & 47.21           \\
Man-Raj           & Raj-WER         & \multicolumn{1}{c}{21.88}             & 16.19           & 15.81            &                    & 15.92           & 16.09           & \textbf{13.19}  & 13.71           \\
Man-Raj           & selected \%s    &                                       & 13.6\% - 8.5\%  & 3.8\% - 12.4\%   &                    & 12.9\% - 8.9\%  & 23.9\% - 7.5\%  & 0.0\% - 100.0\% & 2.7\% - 97.3\%  \\
Man-Raj           & fairness\_\%    &                                       & 4.6             & 1.9              &                    & 4.6             & 7.2             & 0               & \textbf{10.5}   \\
Man-Raj           & mean\_WER       &                                       & 29.37           & 31.52            &                    & 29.17           & \textbf{28.41}  & 31.05           & 30.46           \\
Ass-Hin           & Ass-WER         & \multicolumn{1}{c}{27.06}             & 20.4            & 24.85            &                    & 20.12           & 21.05           & \textbf{17.37}  & 18.32           \\
Ass-Hin           & Hin-WER         & \multicolumn{1}{c}{11.14}             & 9.24            & 9.35             &                    & 9.2             & 9.27            & 11.8            & \textbf{8.71}   \\
Ass-Hin           & selected \%s    &                                       & 17.8\% - 9.3\%  & 1.9\% - 12.3\%   &                    & 16.2\% - 9.8\%  & 15.2\% - 10.0\% & 100.0\% - 0.0\% & 52.6\% - 47.4\% \\
Ass-Hin           & fairness\_\%    &                                       & 6.6             & 0.9              &                    & 6.4             & 6.1             & 0               & \textbf{99.7}   \\
Ass-Hin           & mean\_WER       &                                       & 14.82           & 17.1             &                    & 14.66           & 15.16           & 14.58           & \textbf{13.52}  \\
Raj-Tam           & Raj-WER         & \multicolumn{1}{c}{21.88}             & 16.19           & 15.81            &                    & 15.92           & 16.09           & \textbf{13.83}  & 15.11           \\
Raj-Tam           & Tam-WER         & \multicolumn{1}{c}{12.48}             & 11.84           & 11.94            &                    & 12.05           & 11.92           & \textbf{11.87}  & 12.26           \\
Raj-Tam           & selected \%s    &                                       & 8.5\% - 15.1\%  & 12.4\% - 19.5\%  &                    & 8.9\% - 14.9\%  & 7.5\% - 13.0\%  & 100.0\% - 0.0\% & 79.0\% - 21.0\% \\
Raj-Tam           & fairness\_\%    &                                       & 5.1             & 9.7              &                    & 5.3             & 3.9             & 0               & \textbf{66.4}   \\
Raj-Tam           & mean\_WER       &                                       & 14.02           & 13.88            &                    & 13.98           & 14              & \textbf{12.85}  & 13.68          
\\\hline
\end{tabular}
}
\caption{Doubled-targeted accent adaptation in Indic TTS}
\label{tab:IndicTTS-table-2}
\end{table*}

==> tables/indic/AsmHin.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Eval} & \textbf{Pre} & \textbf{Random} & \textbf{Entropy} & \textbf{PhoneDiv} & \textbf{FL} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FLMI}  \\\hline
{\small ASM-WER ($\mathbf{T\%}$)}   & 27.1 & 20.4 {\small (17.8\%)} & 24.8 {\small (1.9\%)} & 20.7 {\small (17.7\%)} & 20.1 {\small (16.2\%)} & 21.0 {\small (15.1\%)} & \textbf{17.4} {\small (100\%)} & 18.3 {\small (52.6\%)}         \\
{\small HIN-WER ($\mathbf{T\%}$)}   & 11.1 & 9.2 {\small (9.3\%)}   & 9.4 {\small (12.3\%)} & 10.3 {\small (3.6\%)}  & 9.2 {\small (9.8\%)}   & 9.3 {\small (10.0\%)}  & 11.8 {\small (0.0\%)}            & \textbf{8.7} {\small (47.4\%)} \\
{\small Targeted Fairness} &      & 0.07          & 0.01         & 0.03          & 0.06          & 0.06          & 0                       & \textbf{1}            \\
{\small Avg. WER}          &   19.1   & 14.8          & 17.1         & 15.5          & 14.6          & 15.2          & 14.6                    & \textbf{13.5}        \\
\hline
\end{tabular}
}
\caption{Targeting Assamese and Hindi accents (Indic-TTS dataset) on a 2460s budget}
\label{tab:IndicTTS-asm-hin}
\end{table*}

==> tables/indic/AsmMal.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Eval} & \textbf{Pre} & \textbf{Random} & \textbf{Entropy} & \textbf{PhoneDiv} & \textbf{FL} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FLMI}  \\\hline
{\small ASM-WER {\small ($\mathbf{T\%}$)}}          & 27.1 & 20.4 {\small (17.8\%)} & 24.8 {\small (1.9\%)} & 20.7 {\small (17.7\%)} & 20.1 {\small (16.2\%)} & 21.0 {\small (15.1\%)} & 21.1 {\small (24.7\%)}          & \textbf{19.7} {\small (50.6\%)} \\
{\small MAL-WER {\small ($\mathbf{T\%}$)}}           & 19.5 & 16.2 {\small (10.9\%)} & 16.8 {\small (8.6\%)} & 18.4 {\small (3.8\%)}  & 18.7 {\small (8.7\%)}  & 17.5 {\small (4.4\%)}  & \textbf{14.0} {\small (75.3\%)} & 14.7 {\small (49.4\%)}          \\
{\small Targeted Fairness} &      & 0.08          & 0.01         & 0.03          & 0.06          & 0.03          & 0.74                   & \textbf{1}             \\
{\small Avg. WER}          &   23.3   & 18.3          & 20.8         & 19.5          & 19.4          & 19.2          & 17.6                   & \textbf{17.2}    \\
\hline
\end{tabular}
}
\caption{Targeting Assamese and Malayalam accents (Indic-TTS dataset) on a 2460s budget}
\label{tab:IndicTTS-asm-mal}
\end{table*}

% make first row metrics to \small, Targeted Fairness to \smal

==> tables/indic/AsmMan.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Eval} & \textbf{Pre} & \textbf{Random} & \textbf{Entropy} & \textbf{PhoneDiv} & \textbf{FL} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FLMI}  \\\hline
{\small ASM-WER {\small ($\mathbf{T\%}$)}}   & 27.1 & 20.4 {\small (17.8\%)} & 24.8 {\small (1.9\%)} & 20.7 {\small (17.7\%)} & 20.1 {\small (16.2\%)} & 21.0 {\small (15.1\%)} & 17.1 {\small (97.8\%)} & \textbf{17.0} {\small (92.6\%)} \\
{\small MAN-WER {\small ($\mathbf{T\%}$)}}   & 53.1 & 42.5 {\small (13.6\%)} & 47.2 {\small (3.8\%)} & 40.7 {\small (59.0\%)} & 42.4 {\small (12.9\%)} & 40.7 {\small (23.9\%)} & 44.6 {\small (2.2\%)}  & \textbf{42.9} {\small (7.4\%)}  \\
{\small Targeted Fairness} &      & 0.1           & 0            & 0.42          & 0.08          & 0.14          & 0.09          & \textbf{0.27}          \\
{\small Avg. WER}          &   40.1   & 31.4          & 36           & 30.7          & 31.2          & 30.8          & 30.8          & \textbf{30}            \\
\hline
\end{tabular}
}
\caption{Targeting Assamese and Manipuri accents (Indic-TTS dataset) on a 2460s budget}
\label{tab:IndicTTS-ASM-man}
\end{table*}

==> tables/indic/AsmRaj.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Eval} & \textbf{Pre} & \textbf{Random} & \textbf{Entropy} & \textbf{PhoneDiv} & \textbf{FL} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FLMI}  \\\hline
{\small ASM-WER ($\mathbf{T\%}$)}   & 27.1 & 20.4 {\small (17.8\%)} & 24.8 {\small (1.9\%)}  & 20.7 {\small (17.7\%)} & 20.1 {\small (16.2\%)} & 21.0 {\small (15.1\%)} & 25.6 {\small (0.0\%)}            & \textbf{21.2} {\small (25.5\%)} \\
{\small RAJ-WER ($\mathbf{T\%}$)}   & 21.9 & 16.2 {\small (8.5\%)}  & 15.8 {\small (12.4\%)} & 17.2 {\small (4.0\%)}  & 15.9 {\small (8.9\%)}  & 16.1 {\small (7.5\%)}  & \textbf{13.3} {\small (100\%)} & 14.3 {\small (74.5\%)}          \\
{\small Targeted Fairness} &      & 0.06          & 0.01          & 0.03          & 0.06          & 0.05          & 0                       & \textbf{0.76}          \\
{\small Avg. WER}          &   24.5   & 18.3          & 20.3          & 19            & 18            & 18.6          & 19.5           & \textbf{17.8}          \\
\hline
\end{tabular}
}
\caption{Targeting Assamese and Rajasthani accents (Indic-TTS dataset) on a 2460s budget}
\label{tab:IndicTTS-asm-raj}
\end{table*}

==> tables/indic/MalRaj.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Eval} & \textbf{Pre} & \textbf{Random} & \textbf{Entropy} & \textbf{PhoneDiv} & \textbf{FL} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FLMI}  \\\hline
{\small MAL-WER ($\mathbf{T\%}$)}   & 19.5 & 16.2 {\small (10.9\%)} & 16.8 {\small (8.6\%)}  & 18.4 {\small (3.8\%)} & 18.7 {\small (8.7\%)} & 17.5 {\small (4.4\%)} & 15.7 {\small (7.6\%)}           & \textbf{15.0} {\small (21.9\%)} \\
{\small RAJ-WER ($\mathbf{T\%}$)}   & 21.9 & 16.2 {\small (8.5\%)}  & 15.8 {\small (12.4\%)} & 17.2 {\small (4.0\%)} & 15.9 {\small (8.9\%)} & 16.1 {\small (7.5\%)} & \textbf{13.3} {\small (92.4\%)} & 14.3 {\small (78.1\%)}          \\
{\small Targeted Fairness} &      & 0.04          & 0.04          & 0.01         & 0.03         & 0.01         & 0.28                   & \textbf{0.68}          \\
{\small Avg. WER}  &   20.7   & 16.2          & 16.3          & 17.8         & 17.3         & 16.8         & \textbf{14.5}          & 14.6                   \\
\hline
\end{tabular}
}
\caption{Targeting Malayalam and Rajasthani accents (Indic-TTS dataset) on a 2460s budget}
\label{tab:IndicTTS-mal-raj}
\end{table*}

==> tables/indic/ManRaj.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Eval} & \textbf{Pre} & \textbf{Random} & \textbf{Entropy} & \textbf{PhoneDiv} & \textbf{FL} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FLMI}  \\\hline
{\small MAN-WER ($\mathbf{T\%}$)}   & 53.1 & 42.5 {\small (13.6\%)} & 47.2 {\small (3.8\%)}  & 40.7 {\small (59.0\%)} & 42.4 {\small (12.9\%)} & 40.7 {\small (23.9\%)} & 48.9 {\small (0.0\%)}            & \textbf{47.2 {\small (2.7\%)}} \\
{\small RAJ-WER ($\mathbf{T\%}$)}   & 21.9 & 16.2 {\small (8.5\%)}  & 15.8 {\small (12.4\%)} & 17.2 {\small (4.0\%)}  & 15.9 {\small (8.9\%)}  & 16.1 {\small (7.5\%)}  & \textbf{13.2 {\small (100\%)}} & 13.7 {\small (97.3\%)}         \\
{\small Targeted Fairness} &      & 0.05          & 0.02          & 0.09          & 0.05          & 0.07          & 0                       & \textbf{0.11}         \\
{\small Avg. WER}          &  37.5    & 29.4          & 31.5          & 29            & 29.2          & 28.4          & 31                      & \textbf{30.4}         \\
\hline
\end{tabular}
}
\caption{Targeting Manipuri and Rajasthani accents (Indic-TTS dataset) on a 2460s budget}
\label{tab:IndicTTS-man-raj}
\end{table*}

% col

==> tables/indic/RajTam.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Eval} & \textbf{Pre} & \textbf{Random} & \textbf{Entropy} & \textbf{PhoneDiv} & \textbf{FL} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FLMI}  \\\hline
{\small RAJ-WER ($\mathbf{T\%}$)}   & 21.9 & 16.2 {\small (8.5\%)}  & 15.8 {\small (12.4\%)} & 17.2 {\small (4.0\%)} & 15.9 {\small (8.9\%)}  & 16.1 {\small (7.5\%)}  & \textbf{13.8} {\small (100\%)} & 15.1 {\small (79\%)} \\
{\small TAM-WER ($\mathbf{T\%}$)}   & 12.5 & 11.8 {\small (15.1\%)} & 11.9 {\small (19.5\%)} & 12.0 {\small (4.8\%)} & 12.1 {\small (14.9\%)} & 11.9 {\small (13.0\%)} & \textbf{11.9} {\small (0.0\%)}   & 12.3 {\small (21.0\%)} \\
{\small Targeted Fairness} &      & 0.05          & 0.1           & 0.01         & 0.05          & 0.04          & 0                       & \textbf{0.66} \\
{\small Avg. WER}          &   17.2   & 14            & 13.8          & 14.6         & 14            & 14            & \textbf{12.8}           & 13.7         \\
\hline
\end{tabular}
}
\caption{Targeting Rajasthani and Tamil accents (Indic-TTS dataset) on a 2460s budget}
\label{tab:IndicTTS-raj-tam}
\end{table*}

==> tables/l2-2.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{query\_accent} & \textbf{metric} & \multicolumn{1}{c}{\textbf{pretrain}} & \textbf{random} & \textbf{entropy} & \textbf{diversity} & \textbf{FacLoc} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FL2MI}  \\
ARB-CHN                & ARB-WER         & \multicolumn{1}{c}{24.29}             & 22.89           & 23.45            &                    & 23.45           & 22.93           & 20.97           & \textbf{20.29}  \\
ARB-CHN                & CHN-WER         & \multicolumn{1}{c}{30.66}             & 27.08           & 28.29            &                    & 27.54           & 27.83           & 26.31           & \textbf{26.13}  \\
ARB-CHN                & selected \%s    &                                       & 15.4\% - 17.5\% & 17.2\% - 19.0\%  &                    & 15.2\% - 17.2\% & 9.9\% - 13.9\%  & 44.3\% - 31.5\% & 63.5\% - 32.7\% \\
ARB-CHN                & fairness\_\%    &                                       & 10.8            & 13.1             &                    & 10.5            & 5.5             & 55.8            & \textbf{83.1}   \\
ARB-CHN                & mean\_WER       &                                       & 24.98           & 25.87            &                    & 25.49           & 25.38           & 23.64           & \textbf{23.21}  \\
ARB-VTN                & ARB-WER         & \multicolumn{1}{c}{24.29}             & 22.89           & 23.45            &                    & 23.45           & 22.93           & 21.27           & \textbf{20.26}  \\
ARB-VTN                & VTN-WER         & \multicolumn{1}{c}{37.03}             & \textbf{32.79}  & 34.42            &                    & 33.17           & 33.72           & 33.83           & 34.09           \\
ARB-VTN                & selected \%s    &                                       & 15.4\% - 16.8\% & 17.2\% - 16.2\%  &                    & 15.2\% - 17.5\% & 9.9\% - 15.5\%  & 40.8\% - 20.8\% & 74.2\% - 19.8\% \\
ARB-VTN                & fairness\_\%    &                                       & 10.3            & 11.1             &                    & 10.6            & 6.1             & 33.9            & \textbf{58.8}   \\
ARB-VTN                & mean\_WER       &                                       & 27.84           & 28.94            &                    & 28.31           & 28.32           & 27.55           & \textbf{27.18}  \\
CHN-VTN                & CHN-WER         & \multicolumn{1}{c}{30.66}             & 27.08           & 28.29            &                    & 27.54           & 27.83           & 25.88           & \textbf{25.27}  \\
CHN-VTN                & VTN-WER         & \multicolumn{1}{c}{37.03}             & 32.79           & 34.42            &                    & 33.17           & 33.72           & 33.94           & \textbf{32.23}  \\
CHN-VTN                & selected \%s    &                                       & 17.5\% - 16.8\% & 19.0\% - 16.2\%  &                    & 17.2\% - 17.5\% & 13.9\% - 15.5\% & 30.3\% - 15.5\% & 67.3\% - 31.2\% \\
CHN-VTN                & fairness\_\%    &                                       & 11.8            & 12.3             &                    & 12              & 8.6             & 18.8            & \textbf{84}     \\
CHN-VTN                & mean\_WER       &                                       & 29.94           & 31.36            &                    & 30.36           & 30.78           & 29.91           & \textbf{28.75}  \\
ARB-ESP                & ARB-WER         & \multicolumn{1}{c}{24.29}             & 22.89           & 23.45            &                    & 23.45           & 22.93           & 21.17           & \textbf{21.02}  \\
ARB-ESP                & ESP-WER         & \multicolumn{1}{c}{23.44}             & 21.66           & 22.48            &                    & 21.66           & 22.07           & 21              & \textbf{20.98}  \\
ARB-ESP                & selected \%s    &                                       & 15.4\% - 17.6\% & 17.2\% - 23.2\%  &                    & 15.2\% - 16.9\% & 9.9\% - 8.1\%   & 50.8\% - 41.5\% & 43.9\% - 54.4\% \\
ARB-ESP                & fairness\_\%    &                                       & 10.8            & 16               &                    & 10.3            & 3.2             & 84.3            & \textbf{95.5}   \\
ARB-ESP                & mean\_WER       &                                       & 22.28           & 22.96            &                    & 22.56           & 22.5            & 21.08           & \textbf{21}    
\\\hline
\end{tabular}
}
\caption{Doubled-targeted accent adaptation in L2-Artic}
\label{tab:L2Artic-table-2}
\end{table*}

==> tables/l2/ArbChn.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Eval} & \textbf{Pre} & \textbf{Random} & \textbf{Entropy} & \textbf{PhoneDiv} & \textbf{FL} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FLMI}  \\\hline
{\small ARB-WER ($\mathbf{T\%}$)}   & 24.3 & 22.9 {\small (15.4\%)} & 23.4 {\small (17.2\%)} & 22.5 {\small (14.1\%)} & 23.4 {\small (15.2\%)} & 22.9 {\small (9.9\%)}  & 21.0 {\small (44.3\%)} & \textbf{20.3} {\small (63.5\%)} \\
{\small CHN-WER ($\mathbf{T\%}$)}   & 30.7 & 27.1 {\small (17.5\%)} & 28.3 {\small (19.0\%)} & 27.7 {\small (19.6\%)} & 27.5 {\small (17.2\%)} & 27.8 {\small (13.9\%)} & 26.3 {\small (31.5\%)} & \textbf{26.1} {\small (32.7\%)} \\
{\small Targeted Fairness} &      & 0.11          & 0.13          & 0.11          & 0.1           & 0.06          & 0.56          & \textbf{0.83}          \\
{\small Avg. WER}          &   27.5   & 25            & 25.8          & 25.1          & 25.4          & 25.4          & 23.6          & \textbf{23.2}         \\
\hline
\end{tabular}
}
\caption{Targeting Arabic and Chinese accents together (L2-Artic dataset) on a 2460s budget}
\label{tab:l2-arb-chn}
\end{table*}

==> tables/l2/ArbEsp.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Eval} & \textbf{Pre} & \textbf{Random} & \textbf{Entropy} & \textbf{PhoneDiv} & \textbf{FL} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FLMI}  \\\hline
{\small ARB-WER ($\mathbf{T\%}$)}   & 24.3 & 22.9 {\small (15.4\%)} & 23.4 {\small (17.2\%)} & 22.5 {\small (14.1\%)} & 23.4 {\small (15.2\%)} & 22.9 {\small (9.9\%)} & 21.2 {\small (50.8\%)}          & \textbf{21.0} {\small (43.9\%)} \\
{\small ESP-WER ($\mathbf{T\%}$)}   & 23.4 & 21.7 {\small (17.6\%)} & 22.5 {\small (23.2\%)} & 21.7 {\small (18.1\%)} & 21.7 {\small (16.9\%)} & 22.1 {\small (8.1\%)} & \textbf{21.0 {\small (41.5\%)}} & \textbf{21.0} {\small (54.4\%)} \\
Targeted Fairness &      & 0.11          & 0.16          & 0.1           & 0.1           & 0.03         & 0.84                   & \textbf{0.96}          \\
Avg. WER          &      & 22.3          & 23            & 22.1          & 22.5          & 22.5         & 21.1                   & \textbf{21}     \\
\hline
\end{tabular}
}
\caption{Targeting Arabic and Spanish accents together (L2-Artic dataset) on a 2460s budget}
\label{tab:l2-arb-esp}
\end{table*}

==> tables/l2/ArbVtn.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Eval} & \textbf{Pre} & \textbf{Random} & \textbf{Entropy} & \textbf{PhoneDiv} & \textbf{FL} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FLMI}  \\\hline
{\small ARB-WER ($\mathbf{T\%}$)}   & 24.3 & 22.9 {\small (15.4\%)} & 23.4 {\small (17.2\%)} & 22.5 {\small (14.1\%)} & 23.4 {\small (15.2\%)} & 22.9 {\small (9.9\%)}  & 21.3 {\small (40.8\%)}          & \textbf{20.3} {\small (74.2\%)} \\
{\small VTN-WER ($\mathbf{T\%}$)}   & 37   & 32.8 {\small (16.8\%)} & 34.4 {\small (16.2\%)} & 33.6 {\small (17.3\%)} & 33.2 {\small (17.5\%)} & 33.7 {\small (15.5\%)} & \textbf{33.8} {\small (20.8\%)} & 34.1 {\small (19.9\%)}          \\
{\small Targeted Fairness} &      & 0.1           & 0.11          & 0.1           & 0.11          & 0.06          & 0.34                   & \textbf{0.59}          \\
Avg. WER          &   30.6   & 27.8          & 28.9          & 28            & 28.3          & 28.3          & 27.6                   & \textbf{27.2}         \\
\hline
\end{tabular}
}
\caption{Targeting Arabic and Vietnamese accents together (L2-Artic dataset) on a 2460s budget}
\label{tab:l2-arb-vtn}
\end{table*}

==> tables/l2/ChnVtn.tex <==
\setlength\tabcolsep{2pt}

\begin{table*}[!ht]
\centering
\scalebox{0.9}{
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\textbf{Eval} & \textbf{Pre} & \textbf{Random} & \textbf{Entropy} & \textbf{PhoneDiv} & \textbf{FL} & \textbf{LogDet} & \textbf{GCMI}   & \textbf{FLMI}  \\\hline
{\small CHN-WER ($\mathbf{T\%}$)}   & 30.7 & 27.1 {\small (17.5\%)} & 28.3 {\small (19.0\%)} & 27.7 {\small (19.6\%)} & 27.5 {\small (17.2\%)} & 27.8 {\small (13.9\%)} & 25.9 {\small (30.3\%)} & \textbf{25.3} {\small (67.3\%)} \\
{\small VTN-WER ($\mathbf{T\%}$)}   & 37   & 32.8 {\small (16.8\%)} & 34.4 {\small (16.2\%)} & 33.6 {\small (17.3\%)} & 33.2 {\small (17.5\%)} & 33.7 {\small (15.5\%)} & 33.9 {\small (15.5\%)} & \textbf{32.2} {\small (31.2\%)} \\
{\small Targeted Fairness} &      & 0.12          & 0.12          & 0.14          & 0.12          & 0.09          & 0.19          & \textbf{0.84}          \\
{\small Avg. WER}          &   33.8   & 30            & 31.4          & 30.6          & 30.4          & 30.8          & 29.9          & \textbf{28.8}         \\
\hline
\end{tabular}
}
\caption{Targeting Chinese and Vietnamese accents together (L2-Artic dataset) on a 2460s budget}
\label{tab:l2-chn-vtn}
\end{table*}
